Topic Modelling of Swedish Newspaper Articles about Coronavirus: a Case Study using Latent Dirichlet Allocation Method

Topic Modelling (TM) is from the research branches of natural language understanding (NLU) and natural language processing (NLP) that is to facilitate insightful analysis from large documents and datasets, such as a summarisation of main topics and the topic changes. This kind of discovery is getting more popular in real-life applications due to its impact on big data analytics. In this study, from the social-media and healthcare domain, we apply popular Latent Dirichlet Allocation (LDA) methods to model the topic changes in Swedish newspaper articles about Coronavirus. We describe the corpus we created including 6515 articles, methods applied, and statistics on topic changes over approximately 1 year and two months period of time from 17th January 2020 to 13th March 2021. We hope this work can be an asset for grounding applications of topic modelling and can be inspiring for similar case studies in an era with pandemics, to support socio-economic impact research as well as clinical and healthcare analytics. Our data and source code are openly available at https://github. com/poethan/Swed_Covid_TM Keywords: Latent Dirichlet Allocation (LDA); Topic Modelling; Coronavirus; Pandemics; Natural Language Understanding; BERT-topic

==> custom.tex <==
\\bibitem{angelov2020top2vec}
Dimo Angelov. 2020.
\newblock Top2vec: Distributed representations of topics.
\newblock \emph{arXiv preprint arXiv:2008.09470}.

\\bibitem{asmussen2019smart_review_TM}
Claus~Boye Asmussen and Charles M{\o}ller. 2019.
\newblock Smart literature review: a practical topic modelling approach to
  exploratory literature review.
\newblock \emph{Journal of Big Data}, 6(1):1--18.

\bibitem{10.1145/1656274.1656280_KNIME_miner}
Michael~R. Berthold, Nicolas Cebron, Fabian Dill, Thomas~R. Gabriel, Tobias
  K\"{o}tter, Thorsten Meinl, Peter Ohl, Kilian Thiel, and Bernd Wiswedel.
  2009.
\newblock \href {https://doi.org/10.1145/1656274.1656280} {Knime - the konstanz
  information miner: Version 2.0 and beyond}.
\newblock \emph{SIGKDD Explor. Newsl.}, 11(1):26–31.

\\bibitem{Blei_2012ProbTM}
David~M. Blei. 2012.
\newblock \href {https://doi.org/10.1145/2133806.2133826} {Probabilistic topic
  models}.
\newblock \emph{Commun. ACM}, 55(4):77–84.

\\bibitem{blei2006dynamic_TM}
David~M Blei and John~D Lafferty. 2006.
\newblock Dynamic topic models.
\newblock In \emph{Proceedings of the 23rd international conference on Machine
  learning}, pages 113--120.

\bibitem{blei2003latent_LDA}
David~M Blei, Andrew~Y Ng, and Michael~I Jordan. 2003.
\newblock Latent dirichlet allocation.
\newblock \emph{Journal of machine Learning research}, 3(Jan):993--1022.

\\bibitem{boyd2010linguistic_TM}
Jordan Boyd-Graber. 2010.
\newblock \emph{Linguistic extensions of topic models}.
\newblock Princeton University.

\bibitem{brousseaudynamic_archives2019}
Eric Brousseau, Bruno Chaves, and Svitlana Galeshchuk. 2019.
\newblock Dynamic analysis of archives contents: the case of the isnie/sioe
  intellectual history.
\newblock In \emph{SIOE 2019 conference}.

\bibitem{brusselaers2022evaluation_sweden_covid}
Nele Brusselaers, David Steadson, Kelly Bjorklund, Sofia Breland, Jens
  Stilhoff~S{\"o}rensen, Andrew Ewing, Sigurd Bergmann, and Gunnar Steineck.
  2022.
\newblock Evaluation of science advice during the covid-19 pandemic in sweden.
\newblock \emph{Humanities and Social Sciences Communications}, 9(1):1--17.

\bibitem{creutz2021nordic_pandemic_travel}
Katja Creutz, Sofie Berglund, Telli~Bet{\"u}l Kalacan, Giacometti Alberto,
  Kristin~M Haugevik, Ninna~Nyberg S{\o}rensen, Mari~W{\o}ien Meijer, and Axa
  Lares. 2021.
\newblock Nordic cooperation amid pandemic travel restrictions.
\newblock \emph{FIIA report}.

\bibitem{devlin-etal-2019-bert}
Jacob Devlin, Ming-Wei Chang, Kenton Lee, and Kristina Toutanova. 2019.
\newblock \href {https://doi.org/10.18653/v1/N19-1423} {{BERT}: Pre-training of
  deep bidirectional transformers for language understanding}.
\newblock In \emph{Proceedings of the 2019 Conference of the North {A}merican
  Chapter of the Association for Computational Linguistics: Human Language
  Technologies, Volume 1 (Long and Short Papers)}, pages 4171--4186,
  Minneapolis, Minnesota. Association for Computational Linguistics.

\bibitem{fredriksson2022prevalence_covid_dental_sw}
Lars Fredriksson, Andreas Cederlund, My~Murray, Leif Jansson, and Pia Skott.
  2022.
\newblock Prevalence of ongoing or previous sars-cov-2 infection among dental
  personnel--the swedish experience.
\newblock \emph{Acta Odontologica Scandinavica}, pages 1--5.

\bibitem{gerlach2018network_TM}
Martin Gerlach, Tiago~P Peixoto, and Eduardo~G Altmann. 2018.
\newblock A network approach to topic models.
\newblock \emph{Science advances}, 4(7):eaaq1360.

\bibitem{gladkoff-etal-2022-measuring}
Serge Gladkoff, Irina Sorokina, Lifeng Han, and Alexandra Alekseeva. 2022.
\newblock \href {https://aclanthology.org/2022.lrec-1.156} {Measuring
  uncertainty in translation quality evaluation ({TQE})}.
\newblock In \emph{Proceedings of the Thirteenth Language Resources and
  Evaluation Conference}, pages 1454--1461, Marseille, France. European
  Language Resources Association.

\\bibitem{greenwood2008lexical_web_topic}
Mark Greenwood and Goran Nenadic. 2008.
\newblock Lexical profiling of existing web directories to support fine-grained
  topic-focused web crawling.

\bibitem{greenwood2009prioritising_hyperlink_term}
Mark~A Greenwood and Goran Nenadic. 2009.
\newblock \emph{Prioritising Hyperlinks for Topic-Focused Web Crawling using
  Lexical and Terminological Profiling}.
\newblock University of Manchester.

\\bibitem{grootendorst2022bertopic_tf_idf}
Maarten Grootendorst. 2022.
\newblock Bertopic: Neural topic modeling with a class-based tf-idf procedure.
\newblock \emph{arXiv preprint arXiv:2203.05794}.

\\bibitem{han2022overview_mte}
Lifeng Han. 2022.
\newblock An overview on machine translation evaluation.
\newblock \emph{arXiv preprint arXiv:2202.11027}.

\\bibitem{han_gladkoff_metaeval_tutorial2022}
Lifeng Han and Serge Gladkoff. 2022.
\newblock \href {https://github.com/poethan/LREC22_MetaEval_Tutorial}
  {Meta-evaluation of translation evaluation methods: a systematic up-to-date
  overview}.
\newblock In \emph{Tutorial at LREC2022}, Marseille, France.

\\bibitem{han-etal-2020-alphamwe}
Lifeng Han, Gareth Jones, and Alan Smeaton. 2020.
\newblock \href {https://www.aclweb.org/anthology/2020.mwe-1.6} {{A}lpha{MWE}:
  Construction of multilingual parallel corpora with {MWE} annotations}.
\newblock In \emph{Proceedings of the Joint Workshop on Multiword Expressions
  and Electronic Lexicons}, pages 44--57, online. Association for Computational
  Linguistics.

\bibitem{han-etal-2021-chinese}
Lifeng Han, Gareth Jones, Alan Smeaton, and Paolo Bolzoni. 2021.
\newblock \href {https://aclanthology.org/2021.nodalida-main.35} {{C}hinese
  character decomposition for neural {MT} with multi-word expressions}.
\newblock In \emph{Proceedings of the 23rd Nordic Conference on Computational
  Linguistics (NoDaLiDa)}, pages 336--344, Reykjavik, Iceland (Online).
  Link{\"o}ping University Electronic Press, Sweden.

\bibitem{hedman2022dying_covid_sweden}
Christel Hedman, Carl~Johan F{\"u}rst, Birgit~H Rasmussen, Agnes van~der Heide,
  and Maria~EC Schelin. 2022.
\newblock Dying during the covid-19 pandemic in sweden: Relatives’
  experiences of end-of-life care (the co-live study).
\newblock \emph{International Journal of Environmental Research and Public
  Health}, 19(23):16146.

\bibitem{jacobi2016quantitative_journalistic_TM}
Carina Jacobi, Wouter Van~Atteveldt, and Kasper Welbers. 2016.
\newblock Quantitative analysis of large amounts of journalistic texts using
  topic modelling.
\newblock \emph{Digital journalism}, 4(1):89--106.

\bibitem{jaya2022joint_Bayesian_sweden}
IGNM Jaya, Henk Folmer, and Johan Lundberg. 2022.
\newblock A joint bayesian spatiotemporal risk prediction model of covid-19
  incidence, ic admission, and death with application to sweden.
\newblock \emph{The Annals of Regional Science}, pages 1--34.

\bibitem{kovavcevic2012topic_suicide_rule_ML}
Aleksandar Kova{\v{c}}evi{\'c}, Azad Dehghan, John~A Keane, and Goran Nenadic.
  2012.
\newblock Topic categorisation of statements in suicide notes with integrated
  rules and machine learning.
\newblock \emph{Biomedical informatics insights}, 5:BII--S8978.

\\bibitem{kubai2022sweden_covid_image}
Anne Kubai. 2022.
\newblock Sweden’s approach to covid-19 in the context of a poised national
  self-image.
\newblock \emph{Revista Cr{\'\i}tica de Ci{\^e}ncias Sociais}, (128):61--88.

\bibitem{nikolenko2017topic_qualitative}
Sergey~I Nikolenko, Sergei Koltcov, and Olessia Koltsova. 2017.
\newblock Topic modelling for qualitative studies.
\newblock \emph{Journal of Information Science}, 43(1):88--102.

\bibitem{noble2021using_topic_dogs}
Peter-John~M{\"a}ntyl{\"a} Noble, Charlotte Appleton, Alan~David Radford, and
  Goran Nenadic. 2021.
\newblock Using topic modelling for unsupervised annotation of electronic
  health records to identify an outbreak of disease in uk dogs.
\newblock \emph{Plos one}, 16(12):e0260402.

\\bibitem{pashakhanlou2022sweden_corona_public}
Arash~Heydarian Pashakhanlou. 2022.
\newblock Sweden's coronavirus strategy: The public health agency and the sites
  of controversy.
\newblock \emph{World Medical \& Health Policy}, 14(3):507--527.

\\bibitem{piksina2020coronavirus_stock_swedish}
Olga Piksina and Patricia Vernholmen. 2020.
\newblock Coronavirus-related sentiment and stock prices: Measuring sentiment
  effects on swedish stock indices.

\bibitem{qi-etal-2020-stanza_tool}
Peng Qi, Yuhao Zhang, Yuhui Zhang, Jason Bolton, and Christopher~D. Manning.
  2020.
\newblock \href {https://doi.org/10.18653/v1/2020.acl-demos.14} {{S}tanza: A
  python natural language processing toolkit for many human languages}.
\newblock In \emph{Proceedings of the 58th Annual Meeting of the Association
  for Computational Linguistics: System Demonstrations}, pages 101--108,
  Online. Association for Computational Linguistics.

\bibitem{rehurek_lrec_Gensim_topic2010}
Radim {\v R}eh{\r u}{\v r}ek and Petr Sojka. 2010.
\newblock {Software Framework for Topic Modelling with Large Corpora}.
\newblock In \emph{{Proceedings of the LREC 2010 Workshop on New Challenges for
  NLP Frameworks}}, pages 45--50, Valletta, Malta. ELRA.
\newblock \url{http://is.muni.cz/publication/884893/en}.

\\bibitem{rosen2004author_TM}
M~ROSEN-ZVI. 2004.
\newblock The author-topic model for authors and documents.
\newblock In \emph{Proceedings of the 20th conference on Uncertainty in
  artificial intelligence, 2004}, pages 487--494. AUAI Press.

\bibitem{saarentausta2022potential_covid_sweden}
Katariina Saarentausta, Lovisa Ivarsson, Susanne Jacobsson, Bj{\"o}rn Herrmann,
  Martin Sundqvist, and Magnus Unemo. 2022.
\newblock Potential impact of the covid-19 pandemic on the national and
  regional incidence, epidemiology and diagnostic testing of chlamydia and
  gonorrhoea in sweden, 2020.
\newblock \emph{Apmis}, 130(1):34--42.

\bibitem{sarker2018data_twitter_task}
Abeed Sarker, Maksim Belousov, Jasper Friedrichs, Kai Hakala, Svetlana
  Kiritchenko, Farrokh Mehryary, Sifei Han, Tung Tran, Anthony Rios, Ramakanth
  Kavuluru, et~al. 2018.
\newblock Data and systems for medication-related text classification and
  concept normalization from twitter: insights from the social media mining for
  health (smm4h)-2017 shared task.
\newblock \emph{Journal of the American Medical Informatics Association},
  25(10):1274--1283.

\bibitem{SPASIC2014605_2014cancer_mining}
Irena Spasić, Jacqueline Livsey, John~A. Keane, and Goran Nenadić. 2014.
\newblock \href
  {https://doi.org/https://doi.org/10.1016/j.ijmedinf.2014.06.009} {Text mining
  of cancer-related information: Review of current status and future
  directions}.
\newblock \emph{International Journal of Medical Informatics}, 83(9):605--623.

\\bibitem{tong2016text_LDA_TM}
Zhou Tong and Haiyi Zhang. 2016.
\newblock A text mining research based on lda topic modelling.
\newblock In \emph{International conference on computer science, engineering
  and information technology}, pages 201--210.

\bibitem{google2017attention}
Ashish Vaswani, Noam Shazeer, Niki Parmar, Jakob Uszkoreit, Llion Jones,
  Aidan~N. Gomez, Lukasz Kaiser, and Illia Polosukhin. 2017.
\newblock Attention is all you need.
\newblock In \emph{Conference on Neural Information Processing System}, pages
  6000--6010.
